Less than Few: Self-Shot Video Instance Segmentation

The goal of this paper is to bypass the need for labelled examples in few-shot video understanding at run time. While proven effective, in many practical video settings even labelling a few examples appears unrealistic. This is especially true as the level of details in spatio-temporal video understanding and with it, the complexity of annotations continues to increase. Rather than performing few-shot learning with a human oracle to provide a few densely labelled support videos, we propose to automatically learn to find appropriate support videos given a query. We call this self-shot learning and we outline a simple self-supervised learning method to generate an embedding space well-suited for unsupervised retrieval of relevant samples. To showcase this novel setting, we tackle, for the first time, video instance segmentation in a self-shot (and few-shot) setting, where the goal is to segment instances at the pixel-level across the spatial and temporal domains. We provide strong baseline performances that utilize a novel transformer-based model and show that self-shot learning can even surpass few-shot and can be positively combined for further performance gains. Experiments on new benchmarks show that our approach achieves strong performance, is competitive to oracle support in some settings, scales to large unlabelled video collections, and can be combined in a semi-supervised setting.

==> tables/comparison_image_segmentation.tex <==

% have put the below table into comparison_vis.tex

% \begin{table}
% 	\centering
% 	\resizebox{0.8\columnwidth}{!}{%
% 		\begin{tabular}{lrr}
% 			\toprule
% 				&\multicolumn{2}{c}{\textbf{MS-COCO}}\\
% 			\cmidrule(lr){2-3}
% 			& one-shot & five-shot\\
% 			\midrule
% 		Michaelis~\etal~\cite{michaelis2018one} & 14.3 & 16.5\\
% 		Yang~\etal~\cite{yang2021few} & 15.5 & 18.1\\
% 			\textit{\textbf{This paper}} & \textbf{16.2} & \textbf{18.9}\\	
% 			\bottomrule
% 		\end{tabular}%
% 	}
% 	\caption{\textbf{Common image instance segmentation} on the reorganization of MS-COCO dataset of~\cite{michaelis2018one}. The metric is mAP with an overlap threshold of 0.5. We perform better across both one- and five- shot settings.}
% 	\label{tab:comparison_image_segmentation}
% \end{table}

==> tables/temporal_action_detection.tex <==
\begin{table}[t] 
        \centering
        \caption{\textbf{Temporal action localization.} All experiments follow the setups of Yang~\etal~\cite{yang2020localizing} on their Common-Thumos dataset. The metric is video-mAP with an overlap threshold of 0.5. Zhang~\etal~\cite{zhang2020zstad} provides the zero-shot method for the temporal action localization task which can localize the unseen activities in a long untrimmed video based on the label embeddings {\color{red} change format to be 1,5 columns instead. }}
        \label{temporal_action}
         \resizebox{0.7\columnwidth}{!}{
        \begin{tabular}{lrr}
        \toprule
         & \textbf{mAP} & \textbf{Annotations} \\
        \midrule
        0 support in training and testing & 37.2 & 0 \\
        Zero-shot~\cite{zhang2020zstad} & 43.4 & 775 \\
        1 self support (temporal segments from the query video) & 38.6 & 0 \\
        5 self support (temporal segments from the query video) & 39.9 & 0 \\
        1 self support (spatial segments from the query video) & 39.2 & 0 \\
        5 self support (spatial segments from the query video) & 40.7 & 0 \\
        1 self support (\textit{This paper}) & 45.8 & 0 \\
        5 self support (\textit{This paper}) & 47.3 & 0 \\
        1 oracle support & 48.7 & 775 \\
        5 oracle support & 51.9 & 3875 \\
        \bottomrule
        \end{tabular}
        }
\end{table}

==> tables/zero-shot-ablation.tex <==
\begin{table}[t] 
\footnotesize
        \centering
        \caption{\textbf{Self-shot \textit{vs.} zero-shot for Video instance segmentation and temporal action localization.} 
        We compare self-shot vs. zero-shot performances on two datasets and tasks. 
        % For Common-VIS dataset, we follow~\cite{dave2019towards} propose an approach that can segment the moving objects in videos, even ones unseen in training. We use the appearance-based segmentation pipeline of ~\cite{dave2019towards} as the zero-shot baseline. 
        For Temporal action localization, we follow the setups of Yang~\etal~\cite{yang2020localizing} on the Common-Thumos dataset. The metric is video-mAP with an overlap threshold of 0.5}
        \label{temporal_action}
        \begin{tabular}{l  cc c ccc}
        \toprule
        &      \multicolumn{2}{c}{Self-VIS} && \multicolumn{3}{c}{Common-Thumos} \\
        \cmidrule{2-3} \cmidrule{5-7}
        Method & 1 & 5 && 1 & 5 & Num Annot.\\
        \midrule
        0 support in training and testing & \multicolumn{2}{c}{\color{gray}38.6}  && \multicolumn{2}{c}{\color{gray}37.2} & 0\\
        Zero-shot/ spatial augment. support     & 44.9  & 47.8  && 39.2 & 40.7 & 0\\
        Zero-shot/ temporal augment. support     & 44.0  & 46.6  && 38.6 & 39.9 & 0\\
        This paper & ? & ? && ? & ? & ?\\
        %Oracle & 53.2 & 56.6 &&  48.7 & 51.9 & 775/3875 \\
        \bottomrule
        \end{tabular}
\end{table}
